Quo Vadis, HCOMP? A Review of 12 Years of Research at the Frontier of Human Computation and Crowdsourcing

The field of human computation and crowdsourcing has historically studied how tasks can be outsourced to humans. However, many tasks previously distributed to human crowds can today be completed by generative AI with human-level abilities, and concerns about crowdworkers increasingly using language models to complete tasks are surfacing. These developments undermine core premises of the field. In this paper, we examine the evolution of the Conference on Human Computation and Crowdsourcing (HCOMP) - a representative example of the field as one of its key venues - through the lens of Kuhn's paradigm shifts. We review 12 years of research at HCOMP, mapping the evolution of HCOMP's research topics and identifying significant shifts over time. Reflecting on the findings through the lens of Kuhn's paradigm shifts, we suggest that these shifts do not constitute a paradigm shift. Ultimately, our analysis of gradual topic shifts over time, combined with data on the evident overlap with related venues, contributes a data-driven perspective to the broader discussion about the future of HCOMP and the field as a whole.

==> FIG-SENTIMENT.tex <==
\begin{figure*}[!htb]%
\centering%
  \includegraphics[width=.7\textwidth]{figures/sentiment-cloud-boxplot.pdf}%
  \caption{Sentiment in articles at the HCOMP conference over time}%
  \Description{figure description}%
  \label{fig:sentiment}%
\end{figure*}%

==> FIG-TOPIC-BARS.tex <==
%
\begin{figure*}[!htb]%
\centering%
  \includegraphics[width=.75\textwidth]{figures/cluster-ranges-bars-sized-selected.pdf}%
  \caption{Selected HCOMP research topics over time, based on embedding clusters of article titles, as identified by the clustering algorithm HDBSCAN.
  % Note that these topics are only approximations, as some topic clusters lack cohesion.
  Carets denote the number of articles published per year.}%
  \Description{A horizontal bar chart plotting research topics over time.}%
  \label{fig:topics-over-time}%
\end{figure*}%
%
